Adversarial Imitation Learning via Random Search

Developing agents that can perform challenging complex tasks is the goal of reinforcement learning. The model-free reinforcement learning has been considered as a feasible solution. However, the state of the art research has been to develop increasingly complicated techniques. This increasing complexity makes the reconstruction difficult. Furthermore, the problem of reward dependency is still exists. As a result, research on imitation learning, which learns policy from a demonstration of experts, has begun to attract attention. Imitation learning directly learns policy based on data on the behavior of the experts without the explicit reward signal provided by the environment. However, imitation learning tries to optimize policies based on deep reinforcement learning such as trust region policy optimization. As a result, deep reinforcement learning based imitation learning also poses a crisis of reproducibility. The issue of complex model-free model has received considerable critical attention. A derivative-free optimization based reinforcement learning and the simplification on policies obtain competitive performance on the dynamic complex tasks. The simplified policies and derivative free methods make algorithm be simple. The reconfiguration of research demo becomes easy. In this paper, we propose an imitation learning method that takes advantage of the derivative-free optimization with simple linear policies. The proposed method performs simple random search in the parameter space of policies and shows computational efficiency. Experiments in this paper show that the proposed model, without a direct reward signal from the environment, obtains competitive performance on the MuJoCo locomotion tasks.

==> reference.tex <==
@inproceedings{levine2013guided,
  title={Guided policy search},
  author={Levine, Sergey and Koltun, Vladlen},
  booktitle={International Conference on Machine Learning},
  pages={1--9},
  year={2013}
}
@inproceedings{schulman2015trust,
  title={Trust region policy optimization},
  author={Schulman, John and Levine, Sergey and Abbeel, Pieter and Jordan, Michael and Moritz, Philipp},
  booktitle={International Conference on Machine Learning},
  pages={1889--1897},
  year={2015}
}
@article{lillicrap2015continuous,
  title={Continuous control with deep reinforcement learning},
  author={Lillicrap, Timothy P and Hunt, Jonathan J and Pritzel, Alexander and Heess, Nicolas and Erez, Tom and Tassa, Yuval and Silver, David and Wierstra, Daan},
  journal={arXiv preprint arXiv:1509.02971},
  year={2015}
}

@article{oh2018self,
  title={Self-Imitation Learning},
  author={Oh, Junhyuk and Guo, Yijie and Singh, Satinder and Lee, Honglak},
  journal={arXiv preprint arXiv:1806.05635},
  year={2018}
}

@article{nair2015massively,
  title={Massively parallel methods for deep reinforcement learning},
  author={Nair, Arun and Srinivasan, Praveen and Blackwell, Sam and Alcicek, Cagdas and Fearon, Rory and De Maria, Alessandro and Panneershelvam, Vedavyas and Suleyman, Mustafa and Beattie, Charles and Petersen, Stig and others},
  journal={arXiv preprint arXiv:1507.04296},
  year={2015}
}

@inproceedings{mnih2016asynchronous,
  title={Asynchronous methods for deep reinforcement learning},
  author={Mnih, Volodymyr and Badia, Adria Puigdomenech and Mirza, Mehdi and Graves, Alex and Lillicrap, Timothy and Harley, Tim and Silver, David and Kavukcuoglu, Koray},
  booktitle={International conference on machine learning},
  pages={1928--1937},
  year={2016}
}

@inproceedings{ho2016generative,
  title={Generative adversarial imitation learning},
  author={Ho, Jonathan and Ermon, Stefano},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4565--4573},
  year={2016}
}

@article{babaeizadeh2016reinforcement,
  title={Reinforcement learning through asynchronous advantage actor-critic on a gpu},
  author={Babaeizadeh, Mohammad and Frosio, Iuri and Tyree, Stephen and Clemons, Jason and Kautz, Jan},
  journal={arXiv preprint arXiv:1611.06256},
  year={2016}
}

@article{hessel2017rainbow,
  title={Rainbow: Combining improvements in deep reinforcement learning},
  author={Hessel, Matteo and Modayil, Joseph and Van Hasselt, Hado and Schaul, Tom and Ostrovski, Georg and Dabney, Will and Horgan, Dan and Piot, Bilal and Azar, Mohammad and Silver, David},
  journal={arXiv preprint arXiv:1710.02298},
  year={2017}
}

@inproceedings{li2017infogail,
  title={Infogail: Interpretable imitation learning from visual demonstrations},
  author={Li, Yunzhu and Song, Jiaming and Ermon, Stefano},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3812--3822},
  year={2017}
}

@article{horgan2018distributed,
  title={Distributed prioritized experience replay},
  author={Horgan, Dan and Quan, John and Budden, David and Barth-Maron, Gabriel and Hessel, Matteo and Van Hasselt, Hado and Silver, David},
  journal={arXiv preprint arXiv:1803.00933},
  year={2018}
}
@inproceedings{chen2015deepdriving,
  title={Deepdriving: Learning affordance for direct perception in autonomous driving},
  author={Chen, Chenyi and Seff, Ari and Kornhauser, Alain and Xiao, Jianxiong},
  booktitle={2015 IEEE International Conference on Computer Vision (ICCV)},
  pages={2722--2730},
  year={2015},
  organization={IEEE}
}
@inproceedings{dean2012large,
  title={Large scale distributed deep networks},
  author={Dean, Jeffrey and Corrado, Greg and Monga, Rajat and Chen, Kai and Devin, Matthieu and Mao, Mark and Senior, Andrew and Tucker, Paul and Yang, Ke and Le, Quoc V and others},
  booktitle={Advances in neural information processing systems},
  pages={1223--1231},
  year={2012}
}
@misc{rlblogpost,
    title={Deep Reinforcement Learning Doesn't Work Yet},
    author={Irpan, Alex},
    howpublished={\url{https://www.alexirpan.com/2018/02/14/rl-hard.html}},
    year={2018}
}
@article{henderson2017optiongan,
  title={Optiongan: Learning joint reward-policy options using generative adversarial inverse reinforcement learning},
  author={Henderson, Peter and Chang, Wei-Di and Bacon, Pierre-Luc and Meger, David and Pineau, Joelle and Precup, Doina},
  journal={arXiv preprint arXiv:1709.06683},
  year={2017}
}
@incollection{billard2008robot,
  title={Robot programming by demonstration},
  author={Billard, Aude and Calinon, Sylvain and Dillmann, Ruediger and Schaal, Stefan},
  booktitle={Springer handbook of robotics},
  pages={1371--1394},
  year={2008},
  publisher={Springer}
}
@inproceedings{pomerleau1991rapidly,
  title={Rapidly adapting artificial neural networks for autonomous navigation},
  author={Pomerleau, Dean},
  booktitle={Advances in neural information processing systems},
  pages={429--435},
  year={1991}
}
@inproceedings{pomerleau1989alvinn,
  title={Alvinn: An autonomous land vehicle in a neural network},
  author={Pomerleau, Dean A},
  booktitle={Advances in neural information processing systems},
  pages={305--313},
  year={1989}
}
@inproceedings{    
gasil,    
title={Generative Adversarial Self-Imitation Learning},    
author={Anonymous},    
booktitle={Submitted to International Conference on Learning Representations},    
year={2019},    
note={under review}    
}
@article{optiongan,
  title={Optiongan: Learning joint reward-policy options using generative adversarial inverse reinforcement learning},
  author={Henderson, Peter and Chang, Wei-Di and Bacon, Pierre-Luc and Meger, David and Pineau, Joelle and Precup, Doina},
  journal={arXiv preprint arXiv:1709.06683},
  year={2017}
}
@article{ars,
  title={Simple random search provides a competitive approach to reinforcement learning},
  author={Mania, Horia and Guy, Aurelia and Recht, Benjamin},
  journal={arXiv preprint arXiv:1803.07055},
  year={2018}
}
@article{es,
  title={Evolution strategies as a scalable alternative to reinforcement learning},
  author={Salimans, Tim and Ho, Jonathan and Chen, Xi and Sidor, Szymon and Sutskever, Ilya},
  journal={arXiv preprint arXiv:1703.03864},
  year={2017}
}
@article{matyas1965random,
  title={Random optimization},
  author={Matyas, J},
  journal={Automation and Remote control},
  volume={26},
  number={2},
  pages={246--253},
  year={1965}
}
@techreport{nesterov2011random,
  title={Random gradient-free minimization of convex functions},
  author={Nesterov, Yurii and Spokoiny, Vladimir},
  year={2011},
  institution={Universit{\'e} catholique de Louvain, Center for Operations Research and Econometrics (CORE)}
}

@inproceedings{flaxman2005online,
  title={Online convex optimization in the bandit setting: gradient descent without a gradient},
  author={Flaxman, Abraham D and Kalai, Adam Tauman and McMahan, H Brendan},
  booktitle={Proceedings of the sixteenth annual ACM-SIAM symposium on Discrete algorithms},
  pages={385--394},
  year={2005},
  organization={Society for Industrial and Applied Mathematics}
}

@inproceedings{rajeswaran2017towards,
  title={Towards generalization and simplicity in continuous control},
  author={Rajeswaran, Aravind and Lowrey, Kendall and Todorov, Emanuel V and Kakade, Sham M},
  booktitle={Advances in Neural Information Processing Systems},
  pages={6550--6561},
  year={2017}
}

@inproceedings{mao2017least,
  title={Least squares generative adversarial networks},
  author={Mao, Xudong and Li, Qing and Xie, Haoran and Lau, Raymond YK and Wang, Zhen and Smolley, Stephen Paul},
  booktitle={Computer Vision (ICCV), 2017 IEEE International Conference on},
  pages={2813--2821},
  year={2017},
  organization={IEEE}
}

@inproceedings{sorg2010reward,
  title={Reward design via online gradient ascent},
  author={Sorg, Jonathan and Lewis, Richard L and Singh, Satinder P},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2190--2198},
  year={2010}
}

@inproceedings{nagabandi2018neural,
  title={Neural network dynamics for model-based deep reinforcement learning with model-free fine-tuning},
  author={Nagabandi, Anusha and Kahn, Gregory and Fearing, Ronald S and Levine, Sergey},
  booktitle={2018 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={7559--7566},
  year={2018},
  organization={IEEE}
}

@misc{gym,
  Author = {Greg Brockman and Vicki Cheung and Ludwig Pettersson and Jonas Schneider and John Schulman and Jie Tang and Wojciech Zaremba},
  Title = {OpenAI Gym},
  Year = {2016},
  Eprint = {arXiv:1606.01540},
}
@misc{baselines,
  author = {Dhariwal, Prafulla and Hesse, Christopher and Klimov, Oleg and Nichol, Alex and Plappert, Matthias and Radford, Alec and Schulman, John and Sidor, Szymon and Wu, Yuhuai and Zhokhov, Peter},
  title = {OpenAI Baselines},
  year = {2017},
  publisher = {GitHub},
  journal = {GitHub repository},
  howpublished = {\url{https://github.com/openai/baselines}},
}

@inproceedings{mujoco,
  title={Mujoco: A physics engine for model-based control},
  author={Todorov, Emanuel and Erez, Tom and Tassa, Yuval},
  booktitle={Intelligent Robots and Systems (IROS), 2012 IEEE/RSJ International Conference on},
  pages={5026--5033},
  year={2012},
  organization={IEEE}
}
@article{mnih2013playing,
  title={Playing atari with deep reinforcement learning},
  author={Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Graves, Alex and Antonoglou, Ioannis and Wierstra, Daan and Riedmiller, Martin},
  journal={arXiv preprint arXiv:1312.5602},
  year={2013}
}
@article{busoniu2008comprehensive,
  title={A comprehensive survey of multiagent reinforcement learning},
  author={Busoniu, Lucian and Babuska, Robert and De Schutter, Bart},
  journal={IEEE Transactions on Systems, Man, And Cybernetics-Part C: Applications and Reviews, 38 (2), 2008},
  year={2008},
  publisher={IEEE}
}

@inproceedings{lange2012autonomous,
  title={Autonomous reinforcement learning on raw visual input data in a real world application},
  author={Lange, Sascha and Riedmiller, Martin and Voigtlander, Arne},
  booktitle={Neural Networks (IJCNN), The 2012 International Joint Conference on},
  pages={1--8},
  year={2012},
  organization={IEEE}
}

@incollection{kober2012reinforcement,
  title={Reinforcement learning in robotics: A survey},
  author={Kober, Jens and Peters, Jan},
  booktitle={Reinforcement Learning},
  pages={579--610},
  year={2012},
  publisher={Springer}
}

@article{zhu2018dexterous,
  title={Dexterous Manipulation with Deep Reinforcement Learning: Efficient, General, and Low-Cost},
  author={Zhu, Henry and Gupta, Abhishek and Rajeswaran, Aravind and Levine, Sergey and Kumar, Vikash},
  journal={arXiv preprint arXiv:1810.06045},
  year={2018}
}

@article{schulman2017proximal,
  title={Proximal policy optimization algorithms},
  author={Schulman, John and Wolski, Filip and Dhariwal, Prafulla and Radford, Alec and Klimov, Oleg},
  journal={arXiv preprint arXiv:1707.06347},
  year={2017}
}
@article{henderson2017deep,
  title={Deep reinforcement learning that matters},
  author={Henderson, Peter and Islam, Riashat and Bachman, Philip and Pineau, Joelle and Precup, Doina and Meger, David},
  journal={arXiv preprint arXiv:1709.06560},
  year={2017}
}

@article{islam2017reproducibility,
  title={Reproducibility of benchmarked deep reinforcement learning tasks for continuous control},
  author={Islam, Riashat and Henderson, Peter and Gomrokchi, Maziar and Precup, Doina},
  journal={arXiv preprint arXiv:1708.04133},
  year={2017}
}
@inproceedings{ng1999policy,
  title={Policy invariance under reward transformations: Theory and application to reward shaping},
  author={Ng, Andrew Y and Harada, Daishi and Russell, Stuart},
  booktitle={ICML},
  volume={99},
  pages={278--287},
  year={1999}
}

@article{lu2011policy,
  title={Policy invariance under reward transformations for general-sum stochastic games},
  author={Lu, Xiaosong and Schwartz, Howard M and Givigi, Sidney Nascimento},
  journal={Journal of Artificial Intelligence Research},
  volume={41},
  pages={397--406},
  year={2011}
}

@misc{tensorflow,
title={{TensorFlow}: Large-Scale Machine Learning on Heterogeneous Systems},
url={http://tensorflow.org/},
note={Software available from tensorflow.org},
author={
    Mart\'{\i}n~Abadi and
    Ashish~Agarwal and
    Paul~Barham and
    Eugene~Brevdo and
    Zhifeng~Chen and
    Craig~Citro and
    Greg~S.~Corrado and
    Andy~Davis and
    Jeffrey~Dean and
    Matthieu~Devin and
    Sanjay~Ghemawat and
    Ian~Goodfellow and
    Andrew~Harp and
    Geoffrey~Irving and
    Michael~Isard and
    Yangqing Jia and
    Rafal~Jozefowicz and
    Lukasz~Kaiser and
    Manjunath~Kudlur and
    Josh~Levenberg and
    Dan~Man\'{e} and
    Rajat~Monga and
    Sherry~Moore and
    Derek~Murray and
    Chris~Olah and
    Mike~Schuster and
    Jonathon~Shlens and
    Benoit~Steiner and
    Ilya~Sutskever and
    Kunal~Talwar and
    Paul~Tucker and
    Vincent~Vanhoucke and
    Vijay~Vasudevan and
    Fernanda~Vi\'{e}gas and
    Oriol~Vinyals and
    Pete~Warden and
    Martin~Wattenberg and
    Martin~Wicke and
    Yuan~Yu and
    Xiaoqiang~Zheng},
  year={2015},
}
